SoK: Beyond IoT MUD Deployments -- Challenges and Future Directions

Due to the advancement of IoT devices in both domestic and industrial environments, the need to incorporate a mechanism to build accountability in the IoT ecosystem is paramount. In the last few years, various initiatives have been started in this direction addressing many socio-technical concerns and challenges to build an accountable system. The solution that has received a lot of attention in both industry and academia is the Manufacturer Usage Description (MUD) specification. It gives the possibility to the IoT device manufacturers to describe communications needed by each device to work properly. MUD implementation is challenging not only due to the diversity of IoT devices and manufacturer/operator/regulators but also due to the incremental integration of MUD-based flow control in the already existing Internet infrastructure. To provide a better understanding of these challenges, in this work, we explore and investigate the prototypes of three implementations proposed by different research teams and organisations, useful for the community to understand which are the various features implemented by the existing technologies. By considering that there exist some behaviours which can be only defined by local policy, we propose a MUD capable network integrating our User Policy Server(UPS). The UPS provides network administrators and endusers an opportunity to interact with MUD components through a user-friendly interface. Hence, we present a comprehensive survey of the challenges.

==> Feraudo2020a/main.tex <==
\section{Introduction}
Due to the advancement and adoption of smart \iot systems in recent years, billions of sensors and actuator devices from thousands of vendors are connected to the Internet. The data generated from these devices generally have spatial and temporal dimensions, which have more contextual value to their local users than remote users.  However, in many use-cases, the collective data generated by distributed sensors/actuators bring value to their remote users. Furthermore,  the standard Internet protocols and Infrastructures are used to meet the remote access and connectivity requirements. The Internet connectivity not only speeds up the process of advancing new global and remote services, but also make these devices more vulnerable to new security, data, and privacy attacks similar to traditional internet-connected machines. Therefore, to minimise possible threats, \iot deployments need to address various security requirements: authentication, confidentiality, integrity, non-repudiation and availability.

Nevertheless, due to resource constraints and heterogeneity of current IoT devices, deployment of full-fledged security solutions is not possible.  Therefore, smart and distributed solutions are needed. One potential solution is to restrict the traffic communication pattern for these devices so that the attack surface is reduced. In order to simplify things and to bring progress in this direction, manufacturers of \iot devices should take responsibility and authority to provide legibility of the traffic generating from their IoT devices, and end-users, who are also network managers in domestic settings, should have user-friendly tools to analyse, detect and control over their IoT devices. 

Giving manufacturers the responsibility to provide a detailed description of the behaviours of the device, has been investigated~\cite{Cisco2019} and an initiative to formalise specifications by IETF (RFC 8520)~\cite{rfc8520}.   In our work, we present a summary of the current work in this direction and identify many research questions and challenges that need future investigation. Furthermore, we present our solutions to address some of these challenges by focussing on the deployment of manufacturer-provided MUD along with user-defined policies for COTS devices.

\textbf{Contributions:} In this paper, we analyse state-of-the-art MUD deployment scenarios and discuss challenges and shortcoming with each approach. We present the User Policy Server (UPS),  which provides to network administrators and end-users the opportunity to interact with MUD components through a user-friendly interface. However, the proof-of-concept provided presents new challenges that are analysed throughout this paper. Hence, we present a list of future work which we think is a contribution to the research community who are working in this direction.

The rest of the paper is organised as follows. In Section~\ref{section:overview}, we describe an overview of the MUD workflow in a home environment and explain how MUD can isolate the IoT devices from potential external and internal security attacks and provide short descriptions of three MUD deployments. In Section~\ref{findings},  we present current open challenges and their security impacts from our knowledge gained by reviewing the three MUD deployments.  In Section, \ref{challenges}, \ref{oursolutions} and \ref {evaluations}, we list some of the security challenges which could be solved by our solutions and then present our solutions and evaluations in the respective Sections. The related work in this direction so far and future work we discuss in Section~\ref{related} and  \ref{conclusion} respectively.
%----------------------------------------------------------------------------------------
%	SECTION 2
%----------------------------------------------------------------------------------------
\section{MUD overview}\label{section:overview}
According to IETF (RFC 8520)~\cite{rfc8520}, a MUD deployment should consist of three architectural building blocks: (1) The Manufacturer User Description (MUD) file, that is created by the device manufacturer to describe the device and its expected network behaviour. (2) A uniform resource locator (URL), that is used to retrieve the MUD file from a manufacturer's server when a device is added to a home or a small business network. (3)  A mechanism for local network management systems to retrieve the description. The workflow between these components is shown in Fig~\ref{fig:Mudflow}.   In \textcircled{1},  when a device added in the network, it sends MUD-URL with a X.509 certificate or DHCP or LLDP (depending on the implementation).  In \textcircled{2}, the local router  (As Network Access Device (NAD)) sends the MUD-URL to AAA server for authentication of the request. In \textcircled{3}, AAA server sends the authenticated MUD-URL to MUD manager.  The MUD Manager, in case of X.509 authentication, validate the signature and request  (\textcircled{4}) and retrieve MUD file from the manufacturer's file server (\textcircled{5}). The MUD file is a YANG-based JSON file (IETF RFC 7951)~\cite{rfc7951}  signed with a public key signature from the device manufacturer. The MUD manager validates and processes the MUD file and store file locally for until its certificate is valid and generate Access Control Lists (ACL). In \textcircled{6}, the MUD manager sends ACL to NAD. The NAD enforces ACL rules it received from the  MUD manager to all the traffic passing through it. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\textwidth]{images/MUD_workflow.pdf}
    \caption{MUD Workflow.}
    \label{fig:Mudflow}
\end{figure}

From the workflow and the MUD specification, we can conclude that MUD specification has provided enough flexibility and scope to choose different implementations to incorporate requirements of various deployment scenarios. In our work,  we focus on investigating three different implementations of MUD deployments: Cisco proof-the-concept~(PoC) implementation, National Institute of Standards and Technology (NIST)~\cite{nist19, ranganathan2019soft} implementation based on Software Defined Network and  OpenSource MUD~\cite{osMud} developed by a consortium of companies (Cable Labs, Cisco, CTIA, Digicert, ForeScout, Global Cyber Alliance, Patton, and Symantec) in device manufacturing and network security, coordinated by a cybersecurity firm, MasterPeace Solutions. We present a comparison of these implementations in the Table~\ref{mudcompare} and provide brief descriptions in this section. 

\subsection{Cisco MUD PoC}
Cisco proposed (shown in Figure~\ref{fig:Cisco_MUD_workflow})  an open-source proof-of-concept~(PoC) intended to help engineers and users to familiarise with the MUD standard. Therefore, the implementation does not include all the mechanisms typical of MUD environments. Some MUD manager automation is not implemented, and some protocol characteristics are not supported ~\cite{dodson2019securing}. 

As illustrated in Figure~\ref{fig:Cisco_MUD_workflow}, they provide a single device serving as MUD manager and a \textit{FreeRADIUS server} (as a AAA Server) that interfaces with the Catalyst 3850-S switch over TCP/IP.  The DHCP server hosted by the Catalyst 3850-S switch is configured to be MUD enabled, i.e. extract MUD URLs from IPv4 DHCP packets. The deployment provided leverages  DHCP and LLDP as MUD URL emission methods. The Cisco MUD Manager interacts with a FreeRADIUS server to authenticate the MUD URL received from the routers, and uses MongoDB to store policy information. Furthermore, its configuration shows the aim of this PoC, i.e. introducing MUD standards to manufacturer and end-users.
% Previous version
%The Cisco MUD deployment is an open-source proof-of-concept~(PoC) implementation (as shown in Figure~\ref{fig:Cisco_MUD_workflow}) that is intended to introduce advanced users and engineers to the MUD concept. The current version does not provide automated MUD manager implementation, and some protocol features are not supported currently~\cite{dodson2019securing}. The PoC deployment is designed with a single device serving as the MUD manager and \textit{FreeRADIUS server} (as a AAA Server) that interfaces with the  Catalyst 3850-S switch over TCP/IP. The Catalyst 3850-S switch contains a DHCP server that is configured to extract MUD URLs from IPv4 DHCP transactions. In the implementation, DHCP and LLDP are leveraged for sending the MUD URL by the IoT devices. The Cisco MUD Manager is built as a callout from \textit{FreeRADIUS} Server and uses MongoDB to store policy information. The MUD manager is configured from a JSON file that will vary slightly based on the installation. This configuration file provides a number of static bindings and directives as to whether both egress and ingress ACLs should be applied~\cite{dodson2019securing}.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\textwidth]{images/Cisco_MUD_workflow.pdf}
    \caption{Logical Architecture of Cisco MUD implementation. }
    \label{fig:Cisco_MUD_workflow}
\end{figure}{}
Along with the standard MUD implementation, Cisco initial architecture also proposed two additional components, Threat Signalling Server and Update Server.  The requirements for DDoS Open Threat Signaling (DOTS) is described in IETF RFC 8612 ~\cite{rfc8612}.

\subsection{NIST MUD}\label{nistov}
The NIST implementation~\cite{nist19} relies on the Software Defined Networking concept, i.e. data plane and control plane disjunction, and OpenFlow SDN switches. In this deployment, the rules are organised in more than one flow tables by the OpenFlow switch. The SDN controllers manage the rules injection and update in two ways relying on particular times: dynamically, when a packet arrives at the controller, or proactively when the switch connects to the controller.  Ranganathan et al.~\cite{ranganathan2019soft} presented an implementation focusing on achieving rules scalability at SDN switch, by using SDN flow rules in three flow tables. The first two flow tables classify source and destination MAC addresses.
In comparison, the third table implements the MUD policy by introducing rules defined in terms of packet classification metadata assigned in the first two tables. After generating the pipeline described, the packet is finally sent to a table that implements L2Switch flow rules which is provided by another application. The latter forces the implementation to not use general Network ACEs.

% This implementation is based on the concept of Software Defined Networking (SDN) and  uses  OpenFlow SDN switches.   An OpenFlow switch implements flow rules in the data plane by arranging  rules in more than one flow tables.  The SDN  controllers  take the responsibility of inserting and updating the rules dynamically (when a packet arrives at the controller) or proactively when the switch connects to the controller~\cite{nist19}.  Ranganathan et al.~\cite{ranganathan2019soft} presented an implementation using SDN flow rules in three flow tables.  this implementation is focused on achieving scalability of the class-based rules  at SDN switch. The first two flow tables  classify source and destination MAC addresses whereas, the third table implements the MUD Access Control Entries (ACEs) with rules that stated in terms of the packet classification metadata that is assigned in the first two tables. Once this flow pipeline is generated the packet being finally sent to a table that implements L2Switch flow rules which is provided by another application. For these reasons general Network ACEs are not implemented by this model. The implementation highlights are the following:
% \begin{itemize}
%  \item  implements MUD-defined ACLs (including Manufacturer, Controller, Model classes) on SDN Switches. 
%   \item uses IETF published YANG models, thus supports model driven design approach.
%    \item implements DHCP or directly administered MUD profiles;  supports DHCP support without modifications to the DHCP server; all DHCP interactions are handled in the SDN controller.
%    \item supports linear scalability of the rule tables by  supporting $O(N)$ flow rules for $N$ distinct MAC addresses at a SDN switch.
%   \item implements dynamic DNS.
%\end{itemize}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\textwidth]{images/Nist-MudArch.pdf}
    \caption{NIST-MUD Architecture.}
    \label{fig:nist-mudArchitecture}
\end{figure}

\subsection{Open Source MUD}
Open Source MUD (osMUD)~\cite{osMud} is an open-source implementation \cite{osMUDImpl} developed by a consortium of device manufacturing and network security companies. By comparing the architecture shown in Fig. \ref{fig:osMUDArchitecture} with those analysed in previous paragraphs, it is noticeable that the MUD manager directly runs on routers. Thus, only routers that have some characteristics are suitable for this deployment. OsMUD is designed easily build, deploy, and run on Open Wireless Router (OpenWRT) platform, which limits the router choice to only those compliant with this platform. Furthermore, the implementation integrates dnsmasq that extracts from the DHCP packets the MUD-URL, provides network infrastructure services, and is designed to be suitable for resource-constrained routers and firewalls.
%Open Source MUD (osMUD) implementation is developed by a consortium of device manufacturing and network security companies and  implementation source code is maintained at github\footnote{\url{https://github.com/osmud/osmud}}.  The architecture of osMUD is shown in Fig. \ref{fig:osMUDArchitecture}; in the current implementation MUD Manager  is directly run on the router.   The osMUD is currently designed to easily build, deploy, and run on the OpenWRT platform and there is integrations with the \textit{dnsmasq}, that is designed to be lightweight and have a small footprint, suitable for resource constrained routers and firewalls and provides network infrastructure services, such as DNS, DHCP, \textit{router advertisement} and \textit{network boot} for small networks and OpenWRT firewall services~\cite{osMud}. The osMUD could be compiled outside of OpenWRT for most C compatible environments. For running the current implementation outside OpenWRT requires a compatible firewall and a MUD compliant DHCP server which can extract MUD url from the DHCP header packet.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\textwidth]{images/osMudArch.pdf}
    \caption{osMUD Architecture.}
    \label{fig:osMUDArchitecture}
\end{figure}
       
\begin{table*}[t]
 \centering
 \captionof{table}{Comparison of MUD implementations\label{mudcompare}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
\textbf{Implementation} & \textbf{Support} & \textbf{URL via DHCP} & \textbf{URL via LLDP} & \textbf{URL via x509} &  \textbf{URL via  another ways} & \textbf{Component of an AAA system}  & \textbf{Sig Verification}\\ \midrule

Cisco-MUD~& PoC - Cisco Catalyst 3850 & Yes (no DHCPv6) & Yes & No & No & Yes & OpenSSL\\ \\
NIST-MUD~& OpenVSwitch & Yes & No & No & with MAC + MUD & No& No\\ \\
osMUD~& Run on openwrt&dnsmasq& No&No&No&No&OpenSSL\\ 
\midrule
\end{tabular}
}
\end{table*}

%\textbf{N.B.} By observing the specification, it is not mandatory that a mud manager is a component of an Authentication, Authorisation and Accounting system. Conversely, \textit{"a MUD file MUST be signed using CMS as an opaque binary object"}\cite{rfc8520}.\\

%\footnotetext[2]{In this method, the device emits its own MUD URL. The DHCP (UDP) request is sent to the Controller, which then fetches the MUD profile. No configuration is necessary for this to work. However, the Manufactuer web site must be up and running and the device must support issuing a MUR URL as part of the DHCP Request.}
%\footnotetext{Associate MAC address with MUD profile by sending the controller a list of addresses along with associated MUD urls.}

%----------------------------------------------------------------------------------------
%	SECTION 3
%----------------------------------------------------------------------------------------

\section{Findings: Limitations and Security issues}\label{findings}
In this section, we discuss the limitations and security issues of the three prototypes described in the previous section.  We investigated these implementations by setting a test environment in our lab. We understand these implementations are proofs-of-concept and are not fully implemented versions. Still, we thought this is a good starting point to understand the pros and cons of each implementation, which motivates further work in this context. Furthermore, this is the first existing analysis in this direction, which explores the challenges that must be considered during the building of a MUD capable network. 

\subsection{Cisco MUD }
As a proof-of-concept, the main limitations of this deployment regard the MUD Manager configuration. In fact, before the beginning of the MUD Manager, the configuration of DNS resolution service is manually performed by a human operator, which implies to restart the MUD manager process if new settings have been made. The static configuration introduces scalability problems, due to the manual configuration of DNS resolution, and availability problems, because the MUD manager needs to be restarted to pick the new settings made. Thus, Cisco deployment is impractical in real environments.

Another static limit, which regards the implementation itself, involves ACLs management. In particular, all rules, including ingress traffic, i.e. traffic received from external sources to the network and directed to local IoT devices, are static. Consequently, even MUD compliant IoT devices are still vulnerable to attacks originating from external domains, also though the device's MUD file makes it clear that the device is not authorised to receive traffic from that domain. Nevertheless, dynamic rules, including egress traffic, i.e. traffic sent from IoT devices to an external domain, are supported~\cite{dodson2019securing}. Thus, an attacker is not able to establish a TCP connection with the device from an outside domain.
%As a proof-of-concept, the limitations of this implementation are mainly related to the static configuration of the MUD Manager.  The MUD Manager does not invoke a DNS resolution service to automatically resolve the fully qualified domain names (FQDNs), but is performed manually by a human operator before beginning execution of the MUD manager service~\cite{dodson2019securing}. This limitation makes deployment of this implementation in real environments impractical due to the following reasons: (1) Scalability problem due to the manual configuration of DNS resolution. (2) Availability problem due to the fact to add new FQDN address resolutions or change existing ones, the MUD manager process needs to be restarted to pick the new DNS changes from the \textit{JSON} configuration file.  This could also represent a vulnerability because an attacker can exploit the period in which the MUD Manager is not available, to attack an IoT device or steal its identity.
%Furthermore, ingress Dynamic ACLs (DACLs), i.e., the traffic that is received from external sources to the network and directed to local IoT devices, are not supported by this version. Consequently, even if a MUD-capable IoT device's MUD file indicates that the IoT device is not authorized to receive traffic from a particular external domain, the DACL that is needed to prohibit that ingress traffic will not be configured on the switch. Therefore, it will still be vulnerable to attacks originating from that domain, even though the device's MUD file makes it clear that the device is not authorized to receive traffic from that domain. Because egress DACLs, i.e., DACLs that pertain to traffic that is sent from IoT devices to an external domain,  are supported. However, if an attacker is able to get packets to an IoT device from an outside domain, it will not be possible for the attacker to establish a TCP connection with the device from that outside domain, thereby limiting the range of attacks that can be launched against the IoT device~~\cite{dodson2019securing}.

\subsection{NIST MUD}
The SDN based PoC provided by Ranganathan et al. \cite{ranganathan2019soft} presents some issues on packet processing. By following the tables pipeline (section \ref{nistov}), the first rule in MAC address (first tables) classifications stage, which is installed when the switch connects, could allow the packet sending to the controller but not to the next table. Thus, a packet may not proceed in the tables pipeline before it can be classified, which implies performance consequences, i.e. switch failure because no packets from a newly connected device can go through the first table until the rule being installed. The behaviour described may be necessary if strict ACLs are required. However, Ranganathan et al. \cite{ranganathan2019soft}  proposed a  \enquote{relaxed} mode to manage these situations by loosening the ACE definition. In this mode packets can proceed in the pipeline while classification flow rules are being installed, which can result in the violation of the MUD ACEs with the condition that the system will become eventually compliant to the MUD ACEs. These packets could get through before the classification rule being installed at the switch.
%This scheme requires that a packet must be processed at the controller and a rule installed before packet processing may proceed. The first rule in the MAC address classification stage (first two flow tables) that is installed when the switch connects, sends the packet to the controller but not to the next table. Thus, a packet may not proceed in the pipeline before it can be classified. This might be necessary if strict ACL dictated behaviour is required. Still, there are some resultant performance consequences, i.e., a disconnected or failed controller causes a switch failure because no packets from a newly arriving device can get through prior to the classification rule being installed. To address this problem, this implementation loosens up the interpretation of the ACE specification. It defines a \enquote{relaxed} mode of operation where packets can proceed in the pipeline while classification flow rules are being installed. This may result in a few packets being allowed to continue, in violation of the MUD ACEs with the condition that the system will become eventually compliant to the MUD ACEs. Consequently, these packets could get through prior to the classification rule being installed at the switch. This could result in a temporary violation of the ACEs \cite{ranganathan2019soft}.

\subsection{Open Source MUD}
The limits emerging from this implementation regards the deployment requirements. To host the MUD manager, only OpenWRT compliant routers using a particular version of dnsmasq can be employed in this deployment. A valuable solution provided by osMUD developers to run the MUD Manager outside OpenWRT is to compile it in C environments. However, it induces new requirements: it requires to use a compatible firewall and a DHCP server that can extract the MUD-URL from the DHCP header packet for MUD Enabled Devices. Thus, OpenWRT remains the most user-friendly alternative, as a result of availability for the majority of general-purpose routers \cite{openwrtSupported} and making the MUD manager deployment easier. 

Lastly, the current implementation does not have MUD file rules for lateral movement; thus, attackers can progressively move through a network, searching for targeted key data and assets.

%As highlighted in the comparison (Table~\ref{mudcompare}), the current version 0.2.0 of osMUD does not validate the signature across the MUD file. If left unimplemented, this could lead to a serious vulnerability, which a potential attacker could exploit both from external and internal network, some of these attacks are: (1)  intercept the communication between the MUD Manager and the MUD File Server, (2) create its own MUD File, in order to allow the desired communication (i.e. to conduct a dos attack) and  send this file created to the MUD manager, (3)  intercept the communication between the IoT device and the MUD Manager when DHCP or LLDP is used, and (4) change the MUD URL with another one that refers to a MUD File Server that provide MUD File forged by the attacker.  Furthermore, the current implementation does not have MUD file rules for lateral movement, thus attackers can progressively move through a network, searching for targeted key data and assets. These vulnerabilities could be avoided in further versions.

%----------------------------------------------------------------------------------------
%	SECTION 4
%----------------------------------------------------------------------------------------
\section{Security Challenges} \label{challenges}
In this section, we summarise the potential security implications of the three MUD implementations.  None of the implementations uses  X.509 option to emit the MUD URL and provides support through DHCP or LLDP.  Therefore, if a device is compromised, the MUD URL issued through it can potentially be spoofed.  Conversely, it is secure when the device uses the X.509 extension since the MUD URL is added to the certificate by the manufacturer. This means that the MUD URL emitted by an X.509 device can not be spoofed without detection, even if the device is exploited.
Further security issues are related to the MUD Specification itself. It does not provide any inherent security protections to IoT devices themselves. If a device's MUD file permits an IoT device to receive communications from a malicious domain, traffic from that domain can be used to attack the IoT device. Similarly, if the MUD file permits an IoT device to send communications to other domains, and if the IoT device is compromised, it can be used to attack those other domains. Some security considerations to keep in mind by users implementing MUD are provided by the specification \cite{rfc8520} in the \textit{Security Consideration} section. However, we list some additional security challenges which need further addressing:
(1) How to prevent a \iot device from a compromised \iot device's local attack in the local environment.
(2) When MUD signing certificate gets expires while MUD file is still deployed and in function locally; MUD Manager should fetch a newly signed file with signature and updates rules without interrupting the IoT device availability and functionality.
(3) MUD enforced rules does not provide sufficient fine-grained control. Individual users may have their deployment setup with may require additional rules; thus a mechanism to incorporate the user policy to filter traffic to provide more fine-grained control is needed.
(4) How to  incorporate updates from Threat Signalling Server. The further question and investigation in this direction is -  should they go through MUD file or through a generalised common server updates (and filters) for all IoT devices.
 
 \begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{images/MUD_UPS_workflow.pdf}
    \caption{Our setup: osMUD with remote MUD file server and local User Policy Server.}
    \label{fig:osMUDlocal}
\end{figure}

%----------------------------------------------------------------------------------------
%	SECTION 5
%----------------------------------------------------------------------------------------
\section{User Policy Server in a MUD enabled network}\label{oursolutions}
% \af{We further investigate solutions for some of the security issues using Open Source MUD implementation~\cite{osMud}}
In this Section, we present and analyze our solution of problem three listed in the previous Section, which we consider of relative importance. The deployment showed in Figure~\ref{fig:osMUDlocal}, which was used in our testbed, has these main components: (1) OpenWRT router running osMUD Manager (2) Manufacturer MUD file server running remotely and (3) our User Policy Server (UPS) running locally on a local server.
The User Policy Server is a web server based on express framework whose architecture is similar to the Manufacturer MUD File Server (MFS). Deploying this entity gives to an administrator/end-user of an internal network the opportunity to store new MUD Files (hereafter called UPS Files) containing rules more suitable for the network in which MUD is deployed. Thus, a network administrator is now able to interact with all the MUD components using a user-friendly interface. 

It should be noted that by using the same YANG compliant \text{JSON} files and MFS interaction, the UPS does not imply relevant changes on the overall osMUD architecture.  In particular, the osMUD implementation is extended by us in order to incorporate the following workflow (Figure~\ref{fig:osMUDlocal}): (1) MUD Manager retrieves the MUD file from the manufacturer MUD file server; (2) MUD Manager  verify and parse files and generate ACL and insert ACL on Netgear router; (3) MUD Manager asks to the UPS if there is another UPS file for the device; (4) if yes, MUD Manager retrieves the file, verify and parse files and generate ACL and insert ACL on Netgear router. 

The previous steps imply that router hosting osMUD has UPS's certificate and that osMUD implementation can request a further UPS file. We assume that the MUD Manager knows a priori the UPS location. To locate UPS files and make the communication trusted, the device's mac-address is used as UPS file name(e.g. \textit{$<$device-mac-address$>$.json}) and each UPS file is signed by the UPS (as MFS case). After obtaining the UPS file, the MUD Manager can now process it and produce the rules to enforce in the router firewall. At the end of this procedure, the union of manufacturer and administrator rules is performed. This behaviour is appropriate to define either internal communication pattern or more relaxed rules. For example, in voice-based assistant systems (e.g., GoogleHome) case, it is hard for the manufacturer to define a communication pattern that allows all communications that it needs. Thus, the administrator can quickly build new communication patterns for the necessary services.

Nevertheless, the rules union could bring out new challenges: redundancy (limited storage) and conflicting rules (packet filtering performance \cite{firewall}). The former can be easily managed by using a matching technique, e.g. rule to insert with IP tables rules. The latter induces a vital problem that needs to be solved. For example, suppose that the manufacturer's rules (MUD file) allow the communication with two different external hosts, say, ${A}$ and ${B}$, but administrator rules (UPS file) allow only ${A}$ and ${C}$. In our current system, the device for which these rules are defined is allowed to communicate with all three hosts (${A}$, ${B}$ and ${C}$). If a priority system is used and administrator rules have the highest priority, the previous device is able to communicate with only ${A}$ and ${C}$. Both problems are beyond the aim of this work, but they will be considered for future UPS versions. Hence, considering the ability to remove/reversing MUD rules, using UPS needs thoughtful consideration. 

The UPS introduction in a MUD enabled the network to pave the way to new exciting scenarios:

\begin{itemize}
    \item \textbf{Automatic UPS File generation}: Use a tool that automatically generates UPS files (YANG compliant \text{JSON} files) by monitoring the internal traffic ~\cite{MUDGEE}.
    \item \textbf{New MUD File structure for UPS Files}: Extension of current file structure to obtain more restrictive rules such as packet rate, maximum packets, time restrictions, maximum ingress and egress points. To implement this, we require extending osMUD Manager, parsing capabilities, and rule enforcement logic.
    \item \textbf{Publish/subscribe architecture}: it is possible to extend the UPS infrastructure with a publish/subscribe model~\cite{Feraudo2020}, where server becomes the publisher and the router becomes subscriber, in order real time rules upgrade. The server can publish, by understanding the traffic behaviour, new rules that must be inserted in the IP tables of the router. The described architecture requires signature based authentication between the router and server, otherwise an attacker could impersonate the server and insert less restrictive rules.
\end{itemize}

%The User Policy Server is a \textit{restful} server whose architecture is similar to the Manufacturer MUD File Server, it stores other MUD Files (hereafter called UPS Files) and sign them using \textit{openssl}.  The UPS gives the chance to an administrator/end-user of an internal network, to add new rules using YANG compliant \text{JSON} files.  In the UPS, to include new rules for an \iot device, we use MAC address of the \iot device to represent the UPS files, thus  the following nomenclature is being followed:\textit{$<$device-mac-address$>$.json}.  The usage of UPS files, can be useful in different scenarios in which the rules produced by the \textit{manufacturer} mud files, are less restrictive than the one desired by an administrator and end-user. For example, in the internal local communications, it is possible to have malicious actors, which could generate device behaviours not prevented by the manufacturer. Hence, giving the possibility to an administrator to add new rules by using the UPS files, allows to increase the level of security in the local network by exploiting the existing architecture of osMUD.

%To incorporate UPS with osMUD architecture, we extended osMUD implementation to allow us to incorporate following workflow: (1) MUD Manager retrieves the MUD file from the manufacturer MUD file server, (2) MUD Manager  verify and parse files and generate ACL and insert ACL on Netgear router. (3) MUD Manager asks to the UPS if there is another UPS file for the device. (4) If yes, MUD Manager retrieves the file, verify and parse files and generate ACL and insert ACL on Netgear router.
%Thus, at the end of this procedure we have the union of the manufacture rules (MR) and the administrator (AR). 

%Our current architecture as shown in Figure~\ref{fig:osMUDlocal}  generate redundancy of rules, which is not good when we have limited storage. However, this can be simply solved by checking which are the rules already present in the IP tables and avoid to insert the equivalent ones.  The current architecture also lacks in resolving the conflicting rules, for example, the mud file created by the manufacture of an IP camera, allows the communication with two different external hosts, say, ${A}$and ${B}$,  but the UPS file allows only ${A}$ and ${C}$. In our current system, IP camera is allowed communication with all three hosts (${A}$, ${B}$ and ${C}$). But, if we provide UPS rules priority over MUD rules, IP camera should be allowed with only  ${A}$ and ${C}$. By default, all MUD whitelist rules are inserted, so adding new whitelist rules using UPS is easy however, for removing/reversing MUD rules using UPS needs a thoughtful  consideration. Therefore, in this work we  have further investigated  these four  extensions of our architecture:
%\begin{itemize}
%    \item \textbf{Automatic UPS File generation}: Use a tool that automatically generates the YANG compliant \text{JSON} files  by monitoring the internal traffic (\cite{MUDGEE}).
%    \item \textbf{New MUD File structure for UPS Files}: Extension of current file structure to obtain more restrictive rules such as packet rate, maximum packets, time restrictions, maximum ingress and egress points. To implement this, we require extending osMUD Manager, parsing capabilities, and rule enforcement logic.
%    \item \textbf{Publish/subscribe architecture}: it is possible to extend the UPS infrastructure with a publish/subscribe model, where server becomes the publisher and the router becomes subscriber. The server can publish, by understanding the traffic behaviour, new rules that must be inserted in the IP tables of the router. In  this architecture we need signature based authentication between the router and server, otherwise an attacker could impersonate the server and insert less restrictive rules.
 %    \item \textbf{GUI based Policy Engine}: A policy engine, which takes rules from MUD and UPS  and signal users if there are any conflicting rules.
 %   \end{itemize}

\subsection{Evaluations}\label{evaluations}
The system evaluations aim to check the feasibility of running such a system in home routers or small business environments. We run experiments in our lab environment on an OpenWRT compliant Netgear router (model WNDR 3700v2) and an entity that hosts the UPS (MacBook Pro, Intel Core i5 and 8 GB of RAM). To check the system feasibility, the tests are performed by considering the total time spent (latency) by the osMUD Manager in:
\begin{itemize}
    \item retrieving the MUD file;
    \item verifying and storing the file locally at the router;
    \item processing the file and installing the rules.
\end{itemize}
These actions depict the setting time of the rules specified in a MUD file.

The tests consider router in its \textbf{booting stage} that represents the highest overloading phase, because of the aggregation of DHCP requests received from all connected devices (IoT and non-IoT). In case of MUD compliant IoT devices, the osMUD manager processes the MUD-URLs one by one to locate the MUD files. Hence, the file retrieving and processing is sequential. Additionally, to study the worst-case scenario, our tests examine the situation where all the IoT devices are turned on before the router boot process so that all the MUD files need to be retrieved at the same time. For testing purpose, the MUD file server provided by osMUD designers \footnote{https://mudfiles.nist.getyikes.com/} is used.

The osMUD manager, when a MUD compliant IoT device has administrator rules (UPS file), has to repeat the same operations listed above after installing the MUD file rules. It is worth noting that these UPS files are not defined for all the MUD compliant device, but only for devices for which is considered appropriate by an administrator (in our test it is simulated with a random number).

The Fig. \ref{fig:aclTime} illustrates the performance of the osMUD manager in classical (without UPS files) and administrator (with UPS files) environment. Both the tests have been repeated 20 times with a file size range between 2-6K. In the test settings, the UPS file requests and MUD file requests are set as: (1,1), (2,2), (2,4), (3,8), (6,16). The numbers in the brackets (a,b) indicate:  a = number of MUD compliant devices (random), which request for UPS file; b = number of MUD compliant devices.

First of all, by considering only the one device scenario, the performance registered by the osMUD manager in the presence of UPS file is slightly worse than those achieved by the classical MUD environment, as a result of an additional request done to the UPS. Nevertheless, the results obtained are better than expected; the latency average in osMUD with the UPS file is 4.1 seconds compared with 2.9 seconds of osMUD in classical cases, which means in average only 1 second worse. One of the reasons that bring out this result comes from the evidence that requests do not leave the local network, which implies a reduction in the file download time. These results are promising and motivate the usage of a User Policy Server in a MUD deployment.

Secondly, in the ideal environment, the time spent on doing these operations is not linear, as a result of not stable connectivity. However, the time is not exponential, so the number of devices do not carry excessive weight on the performance. This is not true for the administrator environment, in which the time depends on the number of devices requires additional requests. For example, the couple (6,16) reached a spike of 55 seconds, compared with 45 seconds of the ideal environment.

In conclusion, in both cases with 16 devices, the time exceeds more than twice the time spent by 8 devices. The evaluation leads us to think that when the number of devices is over a certain threshold, the router starts to slow its performance, for example, in the case illustrated in Fig. \ref{fig:aclTime} the threshold value can be defined as 8 devices, as a result of the considerable growth reached after this number. The circumstance described represents the worst condition that could occur in case of router failure or unexpected reboot of it. In a steady condition in which at most 2 devices at a time are added, the performance registered are acceptable in both the environment even if both the devices requests an additional UPS file.


%Even though our setup shown in Figure~\ref{fig:osMUDlocal} is a prototype and still in development phase, we performed some of the basic evaluations to check the feasibility of running such systems at a router in home or small  business environment.  We run experiments in our lab environment on  an OpenWRT compliant Netgear router (model WNDR 3700v2)  and compared performance of osMUD~\cite{osMud}  and our solution based on osMUD (shown in Figure~\ref{fig:osMUDlocal}). The tests are performed by considering the time spent (latency calculation) by the MUD Manager (1) retrieving the MUD file, (2) verify and storing the file locally at the router, and (3) processing file and installing rules. The experiment is setup to emulate the router booting phase; during booting phase, router aggregates the dhcp requests from all connected \iot devices in a file. The MUD-URL from the file then processed by MUD Manager one by one to retrieve MUD files. This scenario happens when \iot devices are turned on before the router boot process and thus represent the worst case scenario as all \iot devices MUD files need to be retrieved at the same time. The MUD manager implementation by osMUD retrieves files sequentially from the  MUD file servers. For testing purpose we use MUD file server hosted by osMUD\footnote{https://mudfiles.nist.getyikes.com/}. For UPS, we hosted a local server in our internal network. The size of MUD and UPS files range between 2-6K.
%In our current implementation,  MUD Manager could have repeated twice (osMUD with UPS) all three operations:(1) retrieving the MUD file, (2) verify and storing the file locally at the router, and (3) processing file and installing rules.  

%The figure \ref{fig:acl} illustrates the performance of the router in the osMUD and our work of UPS with osMUD. Both the tests have been repeated 20 times. In our evaluation settings, we set UPS file request and MUD file request as: ${(1,1), (2,2), (2,4), (3,8), (6,16)}$ the numbers in the brackets (a,b) indicate: a = number of devices, which requested for a UPS file;  b = number of devices, which request MUD file.


%Starting from only one device, we can see that the performances registered by osMUD with UPS are a bit worse than the osMUD. This is because of the additional request that must be done to the local server. Nevertheless, the results obtained are better than expected; the mean of latency in  osMUD with UPS is  4.1 seconds as compared with 2.9 seconds of the osMUD, therefore,  in average only 1 second worse. This is also due to the fact, that in our current setup we run UPS server in the local environment, so the download problems are limited to the router bit rate. These results are promising and motivate us to the feasibility of running a User Policy Server to include user rules.

%Overall, the time spent on doing these operations is not linear, because of connectivity that is not completely stable and this can influence the download time. But, at the same time is not exponential, so the number of device does not weigh so much on the performance. This is not true for our model. In fact, in this case all depends on how many devices have an additional mud file. For example, in the case of 16 devices (Figure \ref{fig:acl}) we have 6 devices, which request the additional mud file. This leads to a spike of 55 seconds compared with 45 seconds of the classical model. Furthermore, in both the cases with 16 devices, the time exceeds more then twice the time taken by 8 devices. This leads us to think that when the number of devices is over a threshold, the router starts to be slower.\\

%In conclusion, we can say that the growth becomes exponential after 4 devices. Of course, it represents the worst case situation, due to a router failure or to an unexpected reboot of it. In a steady environment in which we add one or two devices at a time, the performance registered are not bad in both the cases, even if two devices request an additional mud file (Figure \ref{fig:acl}).


\begin{figure}%
	\centering
	\includegraphics[width=0.4\textwidth]{images/acl.pdf}
	\caption{Access Control List (ACL) Rule setting time with osMUD and osMUD with UPS.}
	\label{fig:aclTime}
\end{figure}

%----------------------------------------------------------------------------------------
%	SECTION 6
%----------------------------------------------------------------------------------------

\section{Related Work}\label{related}
The use of MUD as an isolation-based defensive mechanism to restrict traffic generated from the \iot devices is still in its early phase. Therefore, only a few deployment scenarios and proof-of-concept (PoC) implementations currently exist.
Andalibi et al.~\cite{Andalibi2019} proposed extended MUD functionality to include traffic patterns - such as message size, peak-rate and maximum message transmissions within a time-period and proposed to implement those filtering at the fog network firewall. However, the paper does not provide any implementation. Also, it does not provide further details related to how these traffic control lists will be enforced at the fog networks and how this solution will be scalable in a large organization.   Yadav et al.~\cite{Yadav2019a} have proposed the scenario of combining user control policies with MUD to provide fine-grained control of IoT data. This work lacks to provide how to use user-based policies with MUD to control messages directly exchanged with external services.  Ranganathan et al.~\cite{ranganathan2019soft} presented a scalable implementation of the MUD standard on OpenFlow-enabled Software Defined Networking switches and  Hamza et al.~ \cite{Hamza2018a, Hamza2019 } developed machine learning methods to detect volumetric attacks such as DoS, reflective TCP/UDP/ICMP flooding, and ARP spoofing to IoT devices in MUD compliant traffic. Feraudo et al.~\cite{Feraudo2020} presented and evaluated Federated Learning in the MUD compliant Edge Network and showed a use-case of User Policy Server (UPS). Gracia et al.~\cite{Garcia2019} presented a proactive security approach managing secured and automated deployment of IoT devices by using an SDN-enabled security architecture in Industrial IoT settings.  Matheu et al.~\cite{Matheu2020} presented an extended  MUD model with a flexible policy language to express additional aspects, such as data privacy, channel protection, and resource authorization. Afek et al.~\cite{Afek2019}  presented a system built upon the MUD specification to provide IoT security through a VNF deployed within the ISP.  
%\begin{table*}[t]
% \centering
% \captionof{table}{Comparison of MUD deployments\label{muddeployment}}
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{cccccccc}
%\toprule
%\textbf{IResearch} & \textbf{Support} & \textbf{URL via DHCP} & \textbf{URL via LLDP} & \textbf{URL via x509} &  \textbf{URL via  another ways} & \textbf{Component of an AAA system}  & \textbf{Sig Verification}\\ \midrule
%
%Andalibi et al.~\cite{Andalibi2019} & &  & &  &  &  & \\ \\
%Yadav et al.~\cite{Yadav2019a} &  &  &  &  &  & & \\ \\
%Ranganathan et al.~\cite{ranganathan2019soft}&  & &  & & & & \\ 
%Feraudo et al.~\cite{Feraudo2020}&  & &  & & & & \\ 
% Hamza et al.~ \cite{Hamza2018a}&  & &  & & & & \\ 
% Afek et al.~\cite{Afek2019}&  & &  & & & & \\ 
% Gracia et al.~\cite{Garcia2019}&  & &  & & & & \\ 
% Matheu et al.~\cite{Matheu2020}&  & &  & & & & \\ 
% 
%\midrule
%\end{tabular}
%}
%\end{table*}


% The research work investigating the Manufacturer Usage Descriptions (MUD) to control and limit traffic and using it to detect anomaly detection are studied by Hamza et al.~\cite{Hamza2019}.
%Is impact of DDoS on Fog Network is more than the edge network? How does a compromised node at the middle of the network will impact the  whole network and what are the conseqences?


%Network-wide Filtering is not new, and have been used by many research before, such as (1) An Enhanced SDN Firewall for Unstructured Local Network, 
%SDFW: SDN-based Stateful Distributed Firewall
%An SDN-Based Approach to Ward Off LAN Attacks
%https://tools.ietf.org/html/draft-eddy-sdnrg-customer-filters-01
%

%----------------------------------------------------------------------------------------
%	SECTION 7
%----------------------------------------------------------------------------------------
\section{Conclusions and Future works}\label{conclusion}
The MUD specification presents some limits from security and architecture perspectives. There exist some behaviours which can be only defined by local policy, even when using components that are fully MUD compliant. If the default policy provided by the manufacturer is not sufficient or too restrictive for the network standard, user actions are necessary to configure the device according to a different and desired policy. Thus, our work explores the existing MUD implementations and tries to find the most convenient deployment for the general user. Furthermore, our work implements the UPS web server that provides a user-friendly interface needed to interact with the MUD components to modify their default settings when required. The behaviour defined allows building whitelist rules more suitable for the network in which MUD is deployed.

Our future directions will be focused on the extension of the User Policy Server functionalities and on solving implementation inconsistencies concerns, to guarantee a higher level of security. The work we presented in this paper provides useful insight, and we hope the research and development community get benefit from this. Furthermore, this work opens up more discussions before we start adopting these solutions in real deployment scenarios.

%Evidence of that is the fact that is not intended to address network authorisation of those IoT devices that have very broad communication patterns (like Alexa and Google Home). Thus, in this paper, we have proposed a MUD capable network, which integrate osMUD as MUD manager and a User Policy Server as a supervisor of the internal communication. The introduction of an additional supervisor as a threat singnaling servers and user policy based MUD manager that interact directly in the local network, can be used to improve the security level. \\
%Nevertheless, during the development of our proof-of-concept, some architectural and security challenges have been arisen. For example, from the osMUD perspective, there are no checking on the rules redundancy and the difference between DHCP requests from MUD capable devices and from general purpose devices, is not managed; from the User Policy Manager perspective, the introduction of new security features requires changes in the UPS File structure and consequently in the osMUD parser implementation.
%In conclusion, our future directions, considering the security issues not prevented by the MUD specification and the problems described above, will be focused on the extension of the functionalities of the User Profile Server and on solving implementation inconsistency problems, in order to guarantee a higher level of security. The work we presented in this paper provides a useful insight and we hope research and development community get benefit from this. Furthermore, this work opens up more discussions before we start adapting these solutions in the real deployment scenarios.

%\section{Conclusion}

% \section{Acknowledgements}





